Failed Reasoning Traces Tell You What Is Fixable (But Not by Reading Them)

When post-trained language models fail on reasoning problems, the common test-time-scaling response is to spend more compute on additional attempts, and the failed traces play no further role. We argue this discards a crucial signal; some failures come from unlucky sampling, where more rollouts help, while others are structural and resist resampling regardless of budget. We propose that failed traces encode recoverability structure: the inference-time signature of which test-time interventions can rescue a given failure. Three problem-level trajectory features, derived from the structure of available interventions, recover this structure from the distributional signature of failed rollouts, not their text. They cluster failures into stable regimes, characterize the failure topography of different post-training methods ($84.3{\pm}4.3\%$ accuracy, $+20\%$ over a majority-class baseline), and support a training-free routing rule that lifts rescue by $+12.2\%$ on the deployment-relevant Steerable-Hard subset (failures where retry is insufficient and a bounded intervention is reachable). The features and the routing rule transfer across two cross-family probes. The same three features thus convert failed traces from discarded data into a diagnostic object, supporting test-time routing and post-training analysis without training-time or weight-space access.

==> emnlp_table_base_rate_control.tex <==
% AUTO-GENERATED by paper-writing/render_tables.py — do not edit by hand
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}%
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrl}
\toprule
\textbf{Model} & \textbf{N} & \textbf{A} & \textbf{R} & \textbf{R$\cap$A} & \textbf{Base Rate} & \textbf{Overlap} & \textbf{Lift} & \textbf{Hyp.\ $p$} \\
\midrule
SFT 0.6B & 243 & 176 & 119 & 104 & 72.4\% & 87.4\% & 1.21$\times$ & $<$0.001 \\
SFT 4B & 243 & 222 & 99 & 90 & 91.4\% & 90.9\% & 1.00$\times$ & 0.67 \\
\bottomrule
\end{tabular}}

\caption{\textbf{Result 4 overlap reported against ancestor base rate.}
  $N$=total CruxEval problems; $A$=number the ancestor passes (ancestor base rate = $A/N$);
  $R$=DL rescues; $R\cap A$=rescues the ancestor already solved.
  \emph{Overlap} = $R\cap A\,/\,R$; \emph{Lift} = Overlap / Base Rate;
  Hyp.\ $p$ = $P(X \geq R\cap A)$ under a hypergeometric null ($\mathcal{H}_0$: rescues drawn uniformly from the pool).
  SFT 4B base rate is $\sim$91\%---the 90.9\% overlap is not significantly above chance (lift = 1.00$\times$, $p=0.67$). The restoration claim is carried by Result 3's lineage-specificity gap (49.4\% vs.\ 18.2\% on CruxEval), with SFT 0.6B providing supplementary above-chance overlap (lift = 1.21$\times$, $p<0.001$).}
\label{tab:base-rate-control}
\end{table*}


==> emnlp_table_regime_classifier.tex <==
% AUTO-GENERATED by paper-writing/render_tables.py — do not edit by hand
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}%
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccc|c}
\toprule
\textbf{True $\backslash$ Predicted} & \textbf{Dist.\ Source} & \textbf{Geo.\ Local} & \textbf{Unresolved} & \textbf{Non-Sp.\ Local} & \textbf{Samp.\ Recov.} & \textbf{Total} \\
\midrule
Distributed Source & \textbf{5} & 0 & 0 & 0 & 5 & 10 \\
Geometry Local & 0 & \textbf{10} & 0 & 0 & 0 & 10 \\
Unresolved & 0 & 4 & \textbf{1} & 2 & 1 & 8 \\
Non-Specific Local & 0 & 21 & 1 & \textbf{0} & 9 & 31 \\
Sampling Recoverable & 0 & 9 & 0 & 13 & \textbf{3} & 25 \\
\midrule
\textbf{Total Pred.} & 5 & 44 & 2 & 15 & 18 & 84 \\
\bottomrule
\end{tabular}}

\caption{%
\textbf{Regime classifier confusion matrix.}
Rows are true \texttt{winning\_regime} labels (from the operator response ladder);
columns are predicted labels under the hybrid classifier (analytical hard rules for
mechanistically distinctive regimes $+$ \textsc{DecisionTree}(depth~3) for residuals).
Classifier inputs are trajectory-level statistics of per-token logit-distribution
deformation (§\ref{sec:features}), computable from failed rollouts alone ---
no intervention results are used as features.
Leave-one-\emph{(model,task)}-out cross-validation; overall accuracy 22.6\%.
The two mechanistically distinctive regimes --- \textbf{Geometry Local}
($\mathit{Rank\ Misrouting}$; high $J_t^{\mathrm{path}}$, near-constant $V_t$ across $K$)
and \textbf{Distributed Source} ($\mathit{Distributed\ Deformation}$; near-zero
$G_t^{\mathrm{cov}}$, elevated $\sigma(\text{logit\_var})$) --- are identified with
100\% and 50\% per-regime accuracy respectively.
Residual regimes (Non-Specific Local, Sampling Recoverable, Unresolved) overlap
in feature space by construction: they represent the \emph{absence} of a dominant
deformation mechanism rather than a positive signature.%
}
\label{tab:regime-classifier}
\end{table*}

